HetSeq: Distributed GPU Training on Heterogeneous Infrastructure

Modern deep learning systems like PyTorch and Tensorflow are able to train enormous models with billions (or trillions) of parameters on a distributed infrastructure. These systems require that the internal nodes have the same memory capacity and compute performance. Unfortunately, most organizations, especially universities, have a piecemeal approach to purchasing computer systems resulting in a heterogeneous infrastructure, which cannot be used to compute large models. The present work describes HetSeq, a software package adapted from the popular PyTorch package that provides the capability to train large neural network models on heterogeneous infrastructure. Experiments with transformer translation and BERT language model shows that HetSeq scales over heterogeneous systems. HetSeq can be easily extended to other models like image classification. Package with supported document is publicly available at https://github.com/yifding/hetseq.

==> 5_results.tex <==



==> figure/component.tex <==
\begin{tikzpicture}
\begin{scope}
	\node [orangebox, draw=red, ultra thick] (task) at (-3.5,3.2) {\scriptsize\texttt{task.py}};
	\node [orangebox] (train) at (-3.5,1.7) {\scriptsize\texttt{train.py}};
	\node [orangebox] (trainer) at (-3.5,0.2) {\scriptsize\texttt{controller.py}};
\end{scope}

\begin{scope}
	\node [bluebox, draw=red, ultra thick] (model) at (0,4) {\scriptsize\textsf{model}};
	\node [bluebox, draw=red, ultra thick] (dataset) at (0,3.15) {\scriptsize\textsf{dataset}};
	\node [bluebox] (loader) at (0,2.3) {\scriptsize\textsf{data loader}};
	\node [bluebox, draw=red, ultra thick] (opt) at (0,1.45) {\scriptsize\textsf{optimizer}};
	\node [bluebox, draw=red, ultra thick] (sched) at (0,0.6) {\scriptsize\textsf{lr scheduler}};
	\node [bluebox] (check) at (0,-0.25) {\scriptsize\textsf{checkpoint}};
	
	\draw [bluearrow] (train) edge (loader.west);
	\draw [blackarrow] (train) edge (check.west);
	
	\draw [blackarrow] (task) edge (model.170);
	\draw [bluearrow] (task) edge (model.185);
	\draw [orangearrow] (task) edge (model.200);
	\draw [orangearrow] (task) edge (opt.west);
	\draw [blackarrow] (task) edge (dataset);
	\draw [blackarrow] (task) edge (loader);
	
	
	\draw [blackarrow] (trainer) edge (opt);
	\draw [blackarrow] (trainer) edge (sched.195);
	\draw [greenarrow] (trainer) edge (opt.190);
	\draw [greenarrow] (trainer) edge (sched.west);
	\draw [greenarrow] (trainer) edge (check.190);
\end{scope}

\begin{scope}[shift={(0,1.4)}]
	\node (v5) at (-2.35,-2.3) {};
	\node (v6) at (-1.35,-2.3) {};
	\node (v7) at (0.05,-2.3) {};
	\node (v8) at (1.05,-2.3) {};
	\node (v3) at (-4.1,-2.3) {};
	\node (v4) at (-3.1,-2.3) {};
	\node (v1) at (-3,-3.1) {};
	\node (v2) at (-2,-3.1) {};
	\draw [blackarrow] (v1) edge (v2);
	\draw [bluearrow] (v3) edge (v4);
	\draw [orangearrow] (v5) edge (v6);
	\draw [greenarrow] (v7) edge (v8);
	\node [box, draw=red, ultra thick, minimum height=10pt, minimum width=30pt] at (-0.5,-3.1) {};
	\node at (-3.7,-2.65) {\scriptsize\textsf{forward pass}};
	\node at (-1.8,-2.65) {\scriptsize\textsf{backpropagation}};
	\node at (0.45,-2.65) {\scriptsize\textsf{parameter update}};
	\node at (-2.6,-3.5) {\scriptsize\textsf{setup}};
	\node at (-0.4,-3.45) {\scriptsize\textsf{extension module}};
\end{scope}
\end{tikzpicture}

==> figure/pipeline.tex <==
\begin{tikzpicture}

\begin{scope}[shift={(-1.45,2.0)}]
	\node [bluebox] (db1) at (-4.5,1.6) {\textsf{\scriptsize data batch $1$}};
	\node [bluebox] (db2) at (-4.5,1.1) {\textsf{\scriptsize data batch $2$}};
	\node [bluebox] (db3) at (-4.5,0.6) {\textsf{\scriptsize data batch $3$}};
\end{scope}

\begin{scope}[shift={(-0.6,4.0)}]  %  top box
	\node [box, draw=black, minimum width=96pt, minimum height=50pt] (box1) at (-0.175,1.05) {};

	\node [bluebox] (p11) at (-1,1.6) {\scriptsize\textsf{param}$_1$};
	\node [bluebox] (p12) at (-1,1.1) {\scriptsize\textsf{param}$_2$};
	\node [align=right] (pgpu1) at (-2.4,1.8) {\scriptsize\textsf{GPU 1}};
	\node [orangebox] (grad111) at (0.65,1.6) {\scriptsize\textsf{grad}$_{11}$};
	\node [orangebox] (grad112) at (0.65,1.1) {\scriptsize\textsf{grad}$_{12}$};
	
	\node [brownbox] (opt1) at (-1,0.5) {\scriptsize\textsf{opt}$_1$};
	\node [redbox] (sch1) at (0.65,0.5) {\scriptsize\textsf{lr\_sch}$_1$};
	\node [dottedbox] at (0.65,1.35) {};	
	\draw [greenarrow] (opt1) edge[bend left=55] (p11.west);
	\draw [greenarrow] (grad111) edge[bend left=55] (sch1.east);
\end{scope}

\begin{scope}[shift={(-0.6,2.00)}]  % middle box
	\node [box, draw=black, minimum width=96pt, minimum height=50pt] (box2) at (-0.175,1.05) {};

	\node [bluebox] (p21) at (-1,1.6) {\scriptsize\textsf{param}$_1$};
	\node [bluebox] (p22) at (-1,1.1) {\scriptsize\textsf{param}$_2$};
	\node [align=right] (pgpu2) at (-2.4,1.8) {\scriptsize\textsf{GPU 2}};
	\node [orangebox] (grad211) at (0.65,1.6) {\scriptsize\textsf{grad}$_{11}$};
	\node [orangebox] (grad212) at (0.65,1.1) {\scriptsize\textsf{grad}$_{12}$};
	
	\node [brownbox] (opt2) at (-1,0.5) {\scriptsize\textsf{opt}$_2$};
	\node [redbox] (sch2) at (0.65,0.5) {\scriptsize\textsf{lr\_sch}$_2$};
	\node [dottedbox] at (0.65,1.35) {};
	\draw [greenarrow] (opt2) edge[bend left=55] (p21.west);
	\draw [greenarrow] (grad211) edge[bend left=55] (sch2.east);
\end{scope}

\begin{scope}[shift={(-0.6,0.00)}]  % bottom box
	\node [box, draw=black, minimum width=96pt, minimum height=50pt] (box3) at (-0.175,1.05) {};

	\node [bluebox] (p31) at (-1,1.6) {\scriptsize\textsf{param}$_1$};
	\node [bluebox] (p32) at (-1,1.1) {\scriptsize\textsf{param}$_2$};
	\node [align=right] (pgpu3) at (-2.4,1.8) {\scriptsize\textsf{GPU 3}};
	\node [orangebox] (grad311) at (0.65,1.6) {\scriptsize\textsf{grad}$_{11}$};
	\node [orangebox] (grad312) at (0.65,1.1) {\scriptsize\textsf{grad}$_{12}$};
	
	\node [brownbox] (opt3) at (-1,0.5) {\scriptsize\textsf{opt}$_3$};
	\node [redbox] (sch3) at (0.65,0.5) {\scriptsize\textsf{lr\_sch}$_3$};
	\node [dottedbox] at (0.65,1.35) {};
	\draw [greenarrow] (opt3) edge[bend left=55] (p31.west);
	\draw [greenarrow] (grad311) edge[bend left=55] (sch3.east);
\end{scope}

\draw [bluearrow] (db1.east) to (box1.west);
\draw [bluearrow] (db2.east) to (box2.west);
\draw [bluearrow] (db3.east) to (box3.west);

% \node [draw=none, fill=none, inner sep=-5pt, outer sep=-2pt] (n1) at (-3.85,1.4) {};
% \node [draw=none, fill=none, inner sep=-5pt, outer sep=-0.75pt] (n2) at (-3.85,4.88) {};
% \draw [bluearrow] (db1) to (n1) to (n2) to (box1.west);
% 
% \draw [bluearrow] (db2) to (box2);
% 
% \node [draw=none, fill=none, inner sep=-5pt, outer sep=-2pt] (n1) at (-3.85,0.1) {};
% \node [draw=none, fill=none, inner sep=0pt, outer sep=-0.75pt] (n2) at (-3.85,-3.12) {};
% \draw [bluearrow] (db3) to (n1) to (n2) to (box3.west);

\begin{scope}[shift={(-0.3,4)}]  % above
	\node [orangebox] (avg1) at (4,1.6) {\scriptsize\textsf{Avg.loss}};
	\node [bluebox] (l1) at (4,1.1) {\scriptsize\textsf{loss}$_1$};
	\node [bluebox2] at (4,0.6) {\scriptsize\textsf{\# of ins}$_1$};
\end{scope}

\begin{scope}[shift={(-0.3,2)}]  % middle
	\node [orangebox] (avg2) at (4,1.6) {\scriptsize\textsf{Avg.loss}};
	\node [bluebox] (l2) at (4,1.1) {\scriptsize\textsf{loss}$_2$};
	\node [bluebox2] at (4,0.6) {\scriptsize\textsf{\# of ins}$_2$};
\end{scope}

\begin{scope}[shift={(-0.3,0)}]  % bottom
	\node [orangebox] (avg3) at (4,1.6) {\scriptsize\textsf{Avg.loss}};
	\node [bluebox] (l3) at (4,1.1) {\scriptsize\textsf{loss}$_3$};
	\node [bluebox2] at (4,0.6) {\scriptsize\textsf{\# of ins}$_3$};
\end{scope}

\draw [bluearrow] (box1) to (l1);
\draw [bluearrow] (box2) to (l2);
\draw [bluearrow] (box3) to (l3);

\draw [orangearrow] (avg1) to (grad111);
\draw [orangearrow] (avg2) to (grad211);
\draw [orangearrow] (avg3) to (grad311);

\begin{scope}[shift={(3.8,2.0)}]  % last box
	\node [orangebox] (av) at (4,1.6) {\scriptsize\textsf{Avg.loss}};
	\node [bluebox] (tl) at (4,1.1) {\scriptsize\textsf{total loss}};
	\node [bluebox2] (ins) at (4,0.6) {\scriptsize\textsf{\# of ins}};
\end{scope}

\draw [bluearrow] (l1.east) to (tl.170);
\draw [bluearrow] (l2.east) to (tl.west);
\draw [bluearrow] (l3.east) to (tl.190);

\draw [orangearrow] (av.west) to (avg1.east);
\draw [orangearrow] (av.west) to (avg2);
\draw [orangearrow] (av.west) to (avg3.east);
\node [draw=none, outer sep=0pt, inner sep=0pt] (v1) at (2.05,5.8) {};
\node [draw=none, outer sep=0pt,  inner sep=0pt] (v2) at (2.05,3.8) {};
\node [draw=none, outer sep=0pt,  inner sep=0pt] (v3) at (2.05,1.8) {};
\draw [draw=red, thick] (v1) to (v2) to (v3);
\node [draw=none, outer sep=0pt,  inner sep=0pt] (v4) at (0.85,5.8) {};
\node [draw=none, outer sep=0pt, inner sep=0pt] (v5) at (0.85,3.8) {};
\node [draw=none, outer sep=0pt, inner sep=0pt] (v6) at (0.85,1.8) {};
\draw [-*, thick, draw=red, fill=red] (v1) edge (v4);
\draw [-*, thick, draw=red, fill=red] (v2) edge (v5);
\draw [-*, thick, draw=red, fill=red] (v3) edge (v6);

\begin{scope}[shift={(1.05,2.0)}]
	\node (v5) at (-2.35,-2.5) {};
	\node (v6) at (-1.35,-2.5) {};
	\node (v7) at (0.05,-2.5) {};
	\node (v8) at (1.05,-2.5) {};
	\node (v3) at (-4.1,-2.5) {};
	\node (v4) at (-3.1,-2.5) {};
	\node (v1) at (2.35,-2.5) {};
	\node (v2) at (3.35,-2.5) {};
	\draw [-*, thick, draw=red, fill=red] (v1) edge (v2);
	\draw [bluearrow] (v3) edge (v4);
	\draw [orangearrow] (v5) edge (v6);
	\draw [greenarrow] (v7) edge (v8);

	\node at (-3.6,-2.85) {\scriptsize\textsf{{forward}}};
	\node at (-1.85,-2.85) {\scriptsize\textsf{{backpropagation}}};
	\node at (0.45,-2.85) {\scriptsize\textsf{{parameter update}}};
	\node at (2.75,-2.85) {\scriptsize\textsf{{gradient update}}};

\end{scope}
\end{tikzpicture}

==> thesis_proposal.tex <==
\section{Introduction}\label{intro}
%outline:
%1 Deep learning requires lots of computer power.
%2 Only the very biggest can do the models.
%3 Most labs have heterogeneous systems that they try to make work.
%4 We describe how do use these systems for training a giant models.
%5 Our solution performs x better on y setup. and z better on w setup.
%6 One takeaway, small models have better speedup.

% Deep learning community has witnessed rapid growth of powerful neural network model breaking the limit the state-of-art record of general tasks and explore new challenging tasks as well as becoming core part of convenient products in daily life. However, it comes with serious challenges. One of the biggest challenges is the large training time under the capacity limitation of graphics processing unit (GPU). In a typical language model or image classification, a well-performed model requires millions, billions of parameters with similar magnitude of training samples; which ends up with days, weeks and even months of training time. It's common one can only fit very few training instances one time in the GPU, which can also yield an unpleasant underfitting model. 

%1 Deep learning is great but requires lots of computer power.
Deep learning community has witnessed rapid growth of powerful neural network model. Many models have matched or even exceeded human beings in a wide range of areas including image classification,
%cite: vgg, resnet
natural language understanding, 
%cite: tranformer, bert, emo, gpt2, xnet
and multiplayer online battle arena (MOBA) games like defense of the ancients 2 (DOTA2) and  StarCraft II.
%cite: open5 and deepstar/openstar
However, the giant models with millions, billions parameters training on big data requires a high computational capacity. The training process could take days, weeks and even months. There is no surprise that most of the state-of-the-art giant models are proposed by large high-tech company. They even go further to spend large amount of money not only on purchasing the hardware (like CPU, GPU and high performance file system), but also on developing new techniques/platiforms like cloud computing (like AWS by Amazon, Azure by Microsoft),  tensor processing unit (TPU) by Google. NVIDIA has also developed many graphics processing unit (GPU) techniques like half-precision float mixture computation (with volta or touring architecture of NVIDIA GPU) and distributed techniques (like infiniband) which can even scale to build GPU computing center (with thousands of NV-Linked V100 GPUs). Newly developed deep learning platiform, ZeRO \& DeepSpeed by Microsoft, can train models with more than 100 billion parameters. In contrary, most research labs have heterogeneous systems(i.e. GPU work stations) with considerable limited power and hardware commonly have various versions making it hard to apply most newly developed techniques. 

Under this limit, we want to train large models by fully utilizing the resources such that we can reduce the gap to push research forward. Here we describe a general data parallel method to train large models faster on heterogeneous systems (i.e. GPU work stations). Basically, we train a model by splitting training data and distribute different data segments to different GPUs. Each GPU has its individual model and optimizer. Different GPUs communicate about model parameters in feedforward stage and losses just before backpropagation. GPU reduces the training time by performing backpropagation in parallel. Our methods achieve up to $7$ times faster (in 8 GPU work stations with 32 GPUs) comparing to single GPU work station (with 4 GPUs). We observe that relatively smaller model (still as large as millions of parameters) achieves better performance especially scalability. We evaluate our method on language model BERT and translation model Transformer. Our method is highly flexible and can be easily applied to many other large models. We will release our code in the future. 

%4 We describe how do use these systems for training a giant models.
%5 Our solution performs x better on y setup. and z better on w setup.
%6 One takeaway, small models have better speedup.

%example including: microsoft AI, google TPU, NVIDIA GPU computation center. 


\section{Preliminaries}
% Standard training archs look like this. describe tensorflow, pytorch Keras
% They have these pieces
%optimizer, model, how they all fit together
Most neural network (NN) models are built upon popular platforms like TensorFlow, PyTorch and Apache TVM. A standard NN model with backpropagation optimization includes: 
$1.$model. $2.$ dataset and dataloader,
$3.$ optimizer with learning rate scheduler, and $4.$ checkpoint module.  Model is described by a directed acyclic graph (DAG) where nodes represent parameters and edges represent the dependencies between parameters.  Dataset is defined by the actual input of the model while dataloader executes the data loading process. Optimizer acts as a key role to optimize (update) the parameter with gradients. Checkpoint module mainly stores and loads model parameters.

In a typical backpropagation training process, first of all, model is loaded and its parameters are initialized or loaded from parameters' checkpoints of pre-trained model. Then datasets are built and loaded into memory. After that, dataloader loads the corresponding part of datasets, called one $\mathbf{batch}$ to pass to the model. Model gets the data and performs feed forward process to compute its object function. After that, the gradients are obtained by performing backpropagation. For each parameter, pre-defined optimizer takes parameter's partial derivative with respect to object function, corresponding learning rate from learning rate scheduler, and other required factors like gradient history to update the parameter. The whole process including feedforward, backpropagation and parameter update, is called one $\mathbf{step}$. When multiple $\mathbf{steps}$ are finished and all the training data is covered, one $\mathbf{epoch}$ is finished. Finally, when training steps/epochs reach certain threshold or other defined training criteria is reached (i.e. object function, learning rate and etc), the model parameters as well as necessary training status (like optimizer status, learning rate status and etc.) are stored as one checkpoint. 

Researchers have developed many techniques to get better performances,  faster converge, and faster training speed. However, when one model with training settings are decided, many remaining methods are not applicable due to the incompatible hardware and heterogeneous system. 
% Lots of tricks that make these speed up. But alas, they don't solve the basic problems

\section{Distributed GPU training on Heterogeneous Systems}
% Describe each of our pieces - probably keeping same outline as last section
The general idea is utilizing data parallelism across heterogeneous systems by scaling the batch size. For example, if one use four GPUs and each GPU can run a batch with $8$ instances, total batch size of $32$ is achieved. If we scale to $32$ GPUs and total batch size is scaled to be $256$. Without considering any overhead and assume that $100\%$ parallelism is achieved, the training speeds up by $8$ times.  
Because distributed GPU training is performed across heterogeneous systems on big data, we need to revise different parts of the training process to embed distribution mechanism, avoid structure hazard (i.e. memory limitation, GPU memory limitation) and reduce the overhead. In our implementation, each GPU is an individual process and inter-process communication (IPC) is utilized. Our method is built on PyTorch
%add website
and fairseq 
%add website
package.  

%covered parts, ddp in model; nccl, shared file or tcp in communication; all reduce in communication; 


%$1.$model described by a directed acyclic graph (DAG) structure with parameters, $2.$ dataset and dataloader, $3.$ optimizer with learning rate scheduler, and $4.$ checkpoint module. 
We utilize torch.nn.parallel.DistributedDataParallel (DDP)
% add website
as our main basement of model implementation. First of all, we need to build c10d Process Group by spawning one individual process for each single GPU. First process/GPU is called $\mathbf{master}$ which has more responsibilities. We need to know how many GPUs we have in total(called the $\mathbf{world size}$) and index (called $\mathbf{rank}$) for each GPU. We also need to define communication methods. Typically, we use NVIDIA Collective Communications Library (NCCL) as our backend to communicate with either transmission control protocol (TCP) or distributed shared file system. We are introducing the remaining training components in the following sections.
Model initialization is covered in model section, forward pass is covered in dataset \& dataloader section, backward pass and optimization step are covered in optimizer section, and storing and loading checkpoints are covered in the checkpoint section. Other interesting tricks are talked about in the last section. 

\subsection{model}
% Model initialization
After process group is initialized, we can build our model. The model is defined as a child module of \textit{torch.nn.module}, which takes an input tensor (i.e. images or sentences), and output a real number (object function).
%as well as associated numbers like tokens and batch sizes. 
In construction stage, the model in master GPU is initialized, after that, its state dictionary broadcasts to all the other GPUs to make sure that all GPUs share exactly the same parameters. 

\subsection{dataset \& dataloader}
% forward pass
% HDF5, h5py, \_\_getitem\_\_, \_\_len\_\_
% multiple files
Different from typical training on one GPU with relatively small amount of data, distributed training on multiple nodes on multiple GPUs with big data has much more challenges. If data is relatively small, the easy and fast way is to load all the data from disk to memory. In each training step, a chunk of data is selected and concatenated to pass to GPU. However, big data does not fit in memory (with even with 128GB or 256GB memory). Secondly, loading step big data is widely recognized as a bottom neck step. We would like to separate datasets into multiple files which can fully utilize the power of multi-threads in I/O and speed up the preprocessing step by operating shards in parallel. On top of the two previous challenges, the index sampler can be tricky and input can include multiple dependent tensors with different data types (heterogeneous data). In all, we want to find an universal way to I/O arbitrary tensors easily and fast in multiple shards while keeping an easy index manner. 

We select HDF5 wrapped by h5py packages
%add github website
as our main strategy to deal with the challenges. In general,  HDF5 represents Hierarchical Data Formats version 5. It supports self-describing and heterogeneous data in large size. The other benefit is that it can group multiple relative tensors together in a hierarchical manner which can be loaded with multi-processes and multi-threads. We define our dataset class as a child module of $\mathtorch{torch.utils.data.Dataset}$. $\mathtorch{\_\_len\_\_}$ and $\mathtorch{\_\_getitem\_\_}$ function are implemented according to the actual input of the model. It is worthy to mention that the file $\mathbf{OPEN}$ operation should defined inside $\mathtorch{\_\_len\_\_}$ and $\mathtorch{\_\_getitem\_\_}$ instead of $\textit{\_\_init\_\_}$ to support multi-threads loading in PyTorch dataloader. In order to handle multiple files, we add another classes to accumulate the lengths of each file. For a given index referred to one training instance, we can locate the corresponding file and its offset to find desired instance.
\subsubsection{forward pass}
When the lengths of all the files are obtained, we can generate the sampler indices by forming batches which satisfy some criteria like maximum instances in a batch (batch size) and maximum number of tokens in a batch. In a distributed training forward pass, each GPU has separate sampling indices according to its GPU index. Each GPU has its individual data loader to load corresponding data by looking up sampling indices and concatenate data together to form a data batch. When data batch is ready, each GPU calculates its individual object function.  

\subsection{optimizer (with learning rate scheduler)}
Similar to model, each GPU has its individual optimizer as well as learning rate scheduler. Both of them are initialized with the same parameters. In a naive parameter update process, parameters are updated by gradient decent with gradient and a fixed learning rate. In distribution settings, we need to carefully think about the correct gradient decent. Since different GPUs may have different batch sizes and different tokens, the object functions have different weights. Even in a well defined setting, the last step of one epoch often contains partial-filled batches and empty batches. For example, if there are $5$ total instances and batch size is set to $2$. We want to perform distributed training on $4$ GPUs named $A$, $B$, $C$ and $D$. The corresponding data batches are $Batch_A = 2,Batch_B = 2,  Batch_C = 1, Batch_D = 0$ respectively. The $Batch_C$ is half filled while $Batch_D$ is empty. If we take the average or sum directly, we get some error which depends on model and data. Instead, we augment the output by associating it with weight number like batch size and token numbers. After all the GPUs get their output, we take the sum of object function and weight number respectively. Then, we can get the average on the master process and broadcast to all the other processes. 

% backward pass and optimization step
\subsubsection{backward pass and optimization step}
For each GPU, as soon as it gets the average object function, it can perform backpropagation to obtain the gradient for its individual model. However, in order to perform the same parameters update, we need to make sure that each parameter has the same partial derivative across GPUs. $\mathtorch{DistributedDataParallel}$ supports partial backpropagation and gradients synchronizations across GPUs. However, if one GPU has empty batch, how to communicate with other GPUs can be a problem. We give the GPU a dummy batch by taking its very first data batch and setting the gradient to $0$ before backpropagation. In this situation, the example we give which $Batch_D=0$ in the first step can cause error because its first data batch is also empty. Theoretically, it can cause error when the number of batches is less than the number of GPUs. But in reality, it is not a problem since the number of batches is way more than thousands. For each individual GPU, after the backward pass is done, its model gets the same gradient after synchronization. Then optimizer takes the learning rate from the associated learning rate scheduler to update parameters in the model. 

\subsection{checkpoint}
Checkpoint is a key component of the training process. Basically, if we store the entire model structures and parameters, we are able to evaluate our model and perform fine-tuning. Checkpoint also empowers us to train a large model in different phases while keeping the same model architecture but change other settings like batch size, optimizer, learning rate scheduler and etc. We can also stop training and continue training at any checkpoint. Another benefit is that we can record the whole training process by storing multiple checkpoints, we can observe interesting properties and may be able to develop new techniques to obtain better performances. 

In our implementation, master process is responsible to store checkpoints while all the processes will load checkpoint before starting new training from a checkpoint. Except storing model parameters, we also need to store other necessary status including: 1. number of epochs, 2. number of steps, 3. optimizer status (with learning rate scheduler status), 4. random number seed and others. We will briefly talk about how to continue training exactly from a training checkpoint using exactly the same training settings. For other changes, one can redefine part of the settings and replace the old settings before new training. 

When we load a checkpoint and want to perform the training with exactly the same setting. First of all, we need to load model parameters from checkpoint. We also need to load optimizer stats (optimizer parameters, optimizer history and parameter related information) and learning rate scheduler status. The tricky part is dataset \& dataloader checkpoint loading. Even though we know the dataset of our training, but we have no idea how it is splitted and shuffled to feed into different GPUs in the step given by the checkpoint. 
Herein we implement the random number controller with single random number seed but different offsets in different random processes. 
Given a random number seed $S$, we initial all the random seed of all the packages as $S$ (i.e., torch, numpy and etc). Whenever We need to perform necessary random process, we use seed $S + offset$ and set seed back to $S$ afterwards. For example, for a certain epoch number $N$, we perform the shuffle and batch building for the whole dataset with random seed $S + N$. For certain step $P$, we perform shuffle and other random process with random seed $S + N + P$. 
In this manner, we can load the same status by repeating all the random process with exactly the same seed. 

\subsection{other tricks}
\subsubsection{delay update (gradient accumulate)}
Compare to forward pass, backward pass is more expensive which needs to compute gradient for the whole model and update all the parameters by the optimizer. Similar to scale batch size by distribute data across GPUs, we can also scale batch size by performing multiple forward passes before doing backward pass. The object function and associated counters are accumulated within multiple forward pass. After certain pass times exceed certain threshold, it performs backward pass. Delay updates reduce the latency in the backward pass and also help us test our distributed settings. For example, if we implement total batch size = $8$ across $8$ GPUs where each GPU has one instance. The model is too large to increase the batch size. This is exactly equivalent to perform delay updates with update frequency = $8$ on a single GPU. We can observe initial loss function curve to adjust our optimizer to obtain better performances.

\subsubsection{Cython}
Compared to C/C++, python is much slower in many ways. If we are loading and shuffling a giant dataset with billions of instance, it gonna takes a long time to perform python loops. With Cython, one can replace a function in python with much faster running speed. It is widely used to evaluate translation with GLUE score and other loop based expensive computation in natural language processing (NLP) and computer vision (CV).

\subsubsection{prefetch and cache}
Even though we achieve multi-processes and multi-threads, we still need to wait for data loading before each forward pass. When we have a considerable large batch, it takes quite some time and can be a bottom neck of the whole training process. We have considered two techniques to handle large batch data loading latency. One is prefetch. Instead of loading every batch just before forward pass, we can fetch the next batch while we have extra computing power training process of current batch . If we have large memory, we can prefetch multiple batches. The other technique is cache, which is frequently used in computer architecture. We utilize least frequently used (LRU) policy to store the frequent data in the memory. If we use the frequent data, We save much time by loading data from memory instead of hard disk. Due to the big data nature, prefetch is much more powerful and commonly used than cache.


\section{Experiments}
%describe datasets and testing environment. (standard, boring)
We test our methodology on two popular model, (1) Transformer on 2014 De-En dataset and (2) BERT on Wikipedia dataset. We perform our experiments on the Center for Research Computing (CRC) at University of Notre Dame. 
%TODO describe the distributed file system, 
% GPU workstation p100, xp, 1080ti
\subsection{Transformer}
The original transformer
%cite transformer
is published to get better translation result. Indeed, it is an encoder-decoder framework which encodes the whole source language sentence, and produce target language sentence by decoding one word a time. With given a special star token, the decoding operates iteratively, by considering the encoding stat as well as  previous target language sentence, until a special stop token to obtain the whole sentence. For each pair of sentences in the training phase, each token of target language sentence is considered as an individual training instance to be classified by the model. 

\subsubsection{Byte Pair Encoding}
In order to reduce the size of dictionary of tokens, byte pair encoding (BPE). Instead of treating each word as a token, BPE further splits words into sub-words by collecting frequent substring. Given a generated token dictionary, it tokenizes a given words in a greedy manner by looking at the dictionary. If it cannot find certain substring at some point, the whole word is labelled as unknown. The model will use the sub-word dictionary to load and train sub-word embeddings. BPE is widely used in natural language processing (NLP) community but has limitation in messy data (e.g., social media data).

\subsubsection{Multi-head and Scaled Dot-Product Attention}
Given three vector, query $Q$, key $K$ and value $V$, their Scaled Dot-Product Attention as calculated in (Eq.(\ref{dot_attention})). The result can be treated as some way of weighted vector combination of value $V$.
\begin{equation}\label{dot_attention}
    Attention(Q, K, V) = softmax(\frac{QK^{T}}{\sqrt{d_{k}}}V)
\end{equation}

The multi-head means, instead of performing scaled dot-product attention for the whole vectors, we can perform linear layer to split them evenly to multiple parts called muti-head. After performing attention, we can concatenate them together to keep the original dimension.
\begin{align*}\label{multi_attention}
         MultiHead(Q, K, V) &= Concat(head_{1},...,head_{h})W^{O} \\
    \text{where  } head_{i} &= Attention(QW_{i}^{Q},KW_{i}^{K},VW_{i}^{V} )
\end{align*}

In the proposed architecture, attention is used in three places. Self-attention in the encoding blocks, self-attention in the decoding blocks and cross-attention in the decoding blocks. In self-attention, all the vectors equal to hidden states $Q=K=V=hidden\_state$. As for cross-attention, query $Q$ comes from hidden state of known target sentence while both key $K$ and value $V$ comes from the final encoding state from the encoding blocks. 

\subsubsection{Positional Embedding}
Different from other encoder-decoder structure like long-short term memory (LSTM) and gated recurrent unit (GRU), transformer has no positional dependencies. In order to adding positional information, positional embedding (e.g., sine function of position) is added to the word embedding. 


\subsection{BERT}
BERT stands for Bidirectional Encoder Representations from Transformers. BERT applies the encoding structure of original transformer to language model. Different from original definition of language model which predictes next word given previous sentence information, it ``mask""s some of the words in a sentence and tries to fill them by the remaining unmasked words. The task is called mask language model (MLM). Besides, it also introduces next sentence prediction task (NSP) to determine whether two sentences are coherent. BERT is very powerful and flexible to be fine-tuned to many downstream tasks. In general, a sentence (usually formed by two sentence segments) is represented by a sequence of sub-word embeddings to feed into the model and obtain hidden states of each sub-word. The hidden state of starting token is utilized to predict sentence coherence (NSP) while the corresponding masked sub-word tokens are performing sub-word token classification task (MLM).
We are briefly introducing several key components of BERT.
%as well as preprocessing.

\subsubsection{Mask Language Model}
Given a sentence whose total number of sub-words is less than certain threshold (e.g., 128 or 512), a probability (e.g. 15\%) is used to mask some sub-words. For the masked words, 80\% of the time, it is replaced as mask token; 10\% of the time, it is replaced by another random word; and in the rest 10\% of the time, it is kept in the original format.

\subsubsection{Next Sentence Prediction}
If one sentence $S_{1}$ is selected from a paragraph (section) of a related corpus$C_{1}$ (certain Wikipedia page), we want to create next sentence task by concatenated with another sentence. $50\%$ of the time, we add a sentence $S_{2}$ strictly belongs to the related corpus and also shows up after the selected sentence $S_{1}$. For the rest $50\%$ time, we append a random sentence from other corpus $C_{2} != C_{1}$. 

\subsubsection{Segment Embedding}
Besides token embedding and positional embedding mentioned in original transformer architecture, we also want to perform NSP task. We also need to encode the sentence segmentation in the sub-word embedding. We create two extra embedding $Seg_{0}$ and $Seg_{1}$, called segment embedding, to represent two sentence segments. The segment embedding is added to word embedding before any operation. 

\section{Results}
\subsection{Transformer on 2014 de-en dataset}
We evaluate our implementation on Transformer using the original base model on the WMT 2014 English-to-German translation task. The model has $6$ encoder layers and $6$ decoder layers. Hidden state (i.e., dimension of word embedding) is 512 and the number of heads is $8$. Dropout rate is set to $0.1$ and loss function utilizes label smooth cross entropy with $\epsilon = 0.1$. The total number of parameters is about $65M$. We utilize the original Adam optimizer with $\beta_{1} = 0.9$, $\beta_{2} = 0.98$ and $\epsilon = 10−9$, as well as the learning rate scheduler (see E.q. \ref{lr_scheduler_1}). 

\begin{equation} 
\label{lr_scheduler_1}
    lrate = d_{model}^{-0.5} \cdot \min(step\_num^{-0.5}, step\_num \cdot warmup\_steps^{-1.5})
\end{equation}

\begin{table}[] 
\caption[dd]{Transformer results on 2014 English-to-German dataset. Experiments are performed on workstations with four GPUs. We use all GPUs using $1$, $2$, $3$ and $4$ workstations, respectively.}
\label{transformer_experment}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{nodes} & \textbf{GPUs} & \textbf{epochs} & \textbf{steps}  & \textbf{AVG step} & \textbf{training time} & \textbf{BLUE score}                 & \textbf{expansion} & \textbf{speed up} \\ \hline
1              & 4             & 128             & 260,000         & \textbf{0.62s}              & 49.5 hr                      & 25.09, 56.8/30.8/18.9/12.0          & \textbf{1.00}      & 1.00              \\ \hline
2              & 8             & 128             & 130,000         & 0.90s                       & 34.8 hr                      & \textbf{25.57, 57.2/31.2/19.3/12.4} & 0.71               & 1.42              \\ \hline
4              & 16            & 128             & 65,000          & 0.94s                       & 18.7 hr                      & 25.19, 57.1/30.9/18.9/12.1          & 0.66               & 2.64              \\ \hline
8              & 32            & 128             & \textbf{32,500} & 0.98s                 & \textbf{10.3 hr}             & 18.74, 52.2/24.4/13.2/7.5           & 0.60               & \textbf{4.80}     \\ \hline
\end{tabular}%
}
\end{table}

For our experiment, we use the GPU work stations with $4$ GPUs in each work station. For different experiments with different number of work stations, We keep everything the same except for the number of steps. Basically, we want to train on the same data with exactly the same total steps. We keep the one station experiment with $260$K steps and reduce other experiments to the corresponding steps. In other words, the product of number of total GPUs and the number of steps is a constant for each individual experiment. 

In each experiment, we measure the time of each training step, total training time and BLUE score of each trained model. The expansion and speed up calculation is all based on total training time. From table~\ref{transformer_experment}, one can observe that, by employing our method, the training speed increases. The speed up gets $1.42$ when using $2$ nodes, gets $2.64$ when using $4$ nodes, and gets $4.89$ when using $8$ nodes. It's interesting that scaling from $1$ node to $2$ nodes, the average time of each step increases $0.28$s compared to original $0.62$s. In comparison, scaling from $2$ nodes to $4$ nodes or from $4$ nodes to $8$ nodes, the averaging step time increases just $0.04$s. So we want to significantly reduce the training time, we should use more GPUs to reduce the impact of initial cost. 

\subsection{BERT on wikipedia dataset} 
\begin{table}[] \label{bert_experment}
\caption[dd]{BERT on Wikipedia dataset. Experiments are performed on workstations with four GPUs. We use all GPUs using $1$, $2$, $3$ and $4$ workstations, respectively.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{nodes} & \textbf{GPUs} & \textbf{GPU Infomation} & \textbf{length} & \textbf{epochs} & \textbf{steps} & \textbf{AVG step} & \textbf{training time} & \textbf{Training Loss} & \textbf{expansion} & \textbf{speed up} \\ \hline
1              & 4             & XP                      & 32              & 1               & 267,139        & \textbf{2.60s}    & 7.19d                  & 0.026                  & \textbf{1.00}      & 1.00              \\ \hline
2              & 8             & XP*2                    & 32              & 1               & 133,570        & 3.70s             & 5.52d                  & 0.028                  & 0.65               & 1.30              \\ \hline
4              & 16            & P100*4                  & 32              & 1               & 66,785         & 2.79s             & \textbf{2.23d}         & 0.031                  & 0.81               & \textbf{3.22}     \\ \hline
8              & 32            & P100*2+XP+1080TI*5      & 28              & \textless{}1    & 20,825         & 10.74s            & 2.60d                  & 0.046                  & -                  & \textbf{-}        \\ \hline
\end{tabular}%
}
\end{table}
%BERT pipeline
BERT model is quite similar to transformer. Basically, it only uses the transformer encoder part. Instead of passing hidden state of to decoder, it applies both mask language model (MLM) and next sentence prediction (NSP) tasks by further utilizing the hidden states. 

In the training phase, a large corpus is our training data. Originally, it contains Wikipedia and BookCorpus. Since BookCorpus is not available anymore, here we only consider Wikipedia as our training data. A training instance includes several parts, first and more standard is a sequence of tokens. Specifically, this sequence is made by two sentences, $\mathbf{A}$ and $\mathbf{B}$. Each token sequence of each sentence is obtained by running the BPE. Furthermore, A starting token '[CLS]' is added in the start of the token sequence, one '[SEP]' is added between two sentences and another '[SEP]' is added at the end of the token sequence. Secondly, a list of segment sequences with the same length of the token sequence is added to the training instance. For the first sentence $\mathbf{A}$ as well as the starting token '[CLS]' and the '[SEP]' between two sentences is labelled as first segment while the rest tokens are labelled as second segment. Thirdly, an indicator to indicator whether the second sentence $\mathbf{B}$ is the next sentence of first sentence $\mathbf{A}$ is added. At last, partial sub-word tokens are masked in the original token sequence. The masked state and the masked tokens are both stored in the training instance. 

When the model performs training, the model gets the input of a batch of training instances to obtain the corresponding hidden states. Specifically, the training instances are processed to be a sub-word embedding sequence. The word embedding here equals to the sum of token embedding (to be trained, sizes equal to sub-word dictionary), positional embedding and segment embedding (to be trained, sizes $2$). After encoding process, the hidden state of the starting token '[CLS]' is passed to a linear layer and activation function to do a binary classification, to predict whether the second sentence $B$ is the next sentence of the first sentence $A$. The masked sub-word tokens also perform linear layer and activation function to do a multiple classification to predict the masked tokens. The loss function is a combination of the cross entropy of both MLM and NSP classification. 

The BERT model can be fine tuned to perform many NLP related task. Here we only train and measure the training loss on base-BERT which has over $1$ billion parameters. We use Adam optimizer with $\beta_{1} = 0.9$, $\beta_{2} = 0.999$ and $\epsilon = 10−8$. We use the original linear decay learning rate scheduler with maximum learning rate $= 0.0001$, total $1$M steps with the first $10$K steps to warm up. We perform the experiments on the same setting.
%TODO: wait for the new experiments finished, to describe the data we obtain








